Designing Data: Proactive Data Collection and Iteration for Machine Learning

Lack of diversity in data collection has caused significant failures in machine learning (ML) applications. While ML developers perform post-collection interventions, these are time intensive and rarely comprehensive. Thus, new methods to track & manage data collection, iteration, and model training are necessary for evaluating whether datasets reflect real world variability. We present designing data, an iterative approach to data collection connecting HCI concepts with ML techniques. Our process includes (1) Pre-Collection Planning, to reflexively prompt and document expected data distributions; (2) Collection Monitoring, to systematically encourage sampling diversity; and (3) Data Familiarity, to identify samples that are unfamiliar to a model using density estimation. We apply designing data to a data collection and modeling task. We find models trained on ''designed'' datasets generalize better across intersectional groups than those trained on similarly sized but less targeted datasets, and that data familiarity is effective for debugging datasets.

==> 00-abstract.tex <==
Lack of diversity in data collection has caused significant failures in machine learning (ML) applications.
While ML developers perform post-collection interventions, these are time intensive and rarely comprehensive.
Thus, new methods to track \& manage data collection, iteration, and model training are necessary for evaluating whether datasets reflect real world variability.
We present \textit{designing data}, an iterative approach to data collection connecting HCI concepts with ML techniques.
Our process includes (1) Pre-Collection Planning, to reflexively prompt and document expected data distributions; (2) Collection Monitoring, to systematically encourage sampling diversity; and (3) Data Familiarity, to identify samples that are unfamiliar to a model using density estimation.
We apply designing data to a data collection and modeling task. 
We find models trained on ``designed'' datasets generalize better across intersectional groups than those trained on similarly sized but less targeted datasets, and that data familiarity is effective for debugging datasets.
\vspace{-.2cm}

==> 01-intro.tex <==
\section{Introduction}
Curating representative training and testing datasets is fundamental to developing robust, generalizable machine learning (ML) models.
However, understanding what is representative for a specific task is an iterative process. ML practitioners need to change data, models, and their associated processes as they become more familiar with their modeling task, as the state of the world evolves, and as ML products are updated or maintained.
Iteration directed by this evolving understanding seeks to improve model performance, often editing datasets to ensure desired outcomes.
Failure to effectively recognize data quality and coverage needs can lead to biased ML models~\cite{mitchell2020diversity}.
Such failures are responsible for the perpetuation of systemic power and access differentials and the deployment of inaccessible or defective product experiences.
Yet building representative datasets is an arduous, historically difficult undertaking~\cite{tayi1998examining, 49953} that relies on the efficacy of human-specified data requirements.

To ensure a dataset covers all, or as many, characteristics as possible, specifications must be the result of a comprehensive enumeration of possible dimensions---an open and hard problem that few have practically grappled with in the context of ML. Further contributing to this difficulty is the realization that it is not enough for the training datasets to be aligned with expected distributions: they must also include enough examples from conceptually harder or less common categories if said categories are to be learned~\cite{asudeh2019assessing}. Failure to sufficiently consider both the critical dimensions of data and their relative complexity can have troubling consequences. Instances of such missteps span issues of justice, healthcare, hiring practices, voice and face recognition, and loan qualifications, wherein biases of data and algorithms limit technological use and cause harm ~\cite{buolamwini2018gender,asudeh2019assessing,palanica2019you,angwin2016machine,noble2018algorithms}. Yet understanding these data requirements even after training is difficult; knowing them \textit{a priori} is exceptionally so.

Rather than emphasize tools that enable better collection and data iteration practices---that \emph{design better data}---research in fairness and machine learning has largely focused on prescriptive ``how-to'' frameworks,  definitions of fairness, and post-collection analysis techniques~\cite{amershi2019guidelines, yang2020towards}. While there are exceptions to this~\cite{hohman2020understanding}, the hidden technical debt~\cite{sculley2015hidden} accumulated from poor data design remains an under explored space. To reduce this technical debt and encourage diverse datasets, methods of externalizing \footnote{For example, documenting design decisions and communicating the evolving state of the data.} data collection, iteration, and training are necessary checks for ensuring datasets reflect diverse experiences and are robust when deployed in real-world models. 

\textbf{Contributions}   We present \emph{designing data}, an iterative, bias mitigating approach to data planning, collection, and ML development; we implement this approach in an interactive dashboard that scaffolds each step for practitioner use. 
Motivated by 24 formative interviews \ref{sec:informal}, designing data is a structured, holistic parallel to the current standards for developing production-quality datasets~\cite{hohman2020understanding}. Each step proactively introduces interventions to improve models prior to deployment: 
\begin{enumerate}
    \item \emph{\textbf{Pre-Collection Planning}} prioritizes reflexive consideration for domain and data needs prior to modeling, documents expected distributions of attributes, and highlights potential biases through questions related to class or characteristic representation within data. 
    \item \emph{\textbf{Collection Monitoring}} communicates insight into dataset evolution, allowing users to make targeted adjustments to collection processes based on new insight or disparities between expected distributions and existing data. 
    \item \emph{\textbf{Data Familiarity}} borrows from Out-of-Distribution (OOD) methodologies to identify data that a model perceives as unfamiliar, creating new directives for data and model iteration. 
\end{enumerate}
    
    
 


We demonstrate designing data's effectiveness through a case study using inertial measurement units (IMU) data--time series data representing X, Y, \& Z positioning--to classify hand position while texting. First, we collected data iteratively, using Pre-Collection Planning and Monitoring steps to build a diverse dataset. Then, we use leave-one-out cross-validation to evaluate how these initial steps  influence performance. Finally, we evaluate familiarity to first debug a dataset, then to direct collection efforts. Each step is centralized within a dashboard. We find models trained on highly diverse data outperform those trained on less diverse data across intersectional groups.


\begin{figure}
  \centering
  \vspace{-.7cm}
  \includegraphics[width=1.0\textwidth]
  {figures/new_overview.pdf}
  \caption{
\textit{Designing data} includes (I) \textbf{Pre-Collection Planning}, (II) \textbf{Collection Monitoring}, \& (III)\textbf{ Data Familiarity}. Each supplements the other, and should be used iteratively.
  \vspace{-.7cm}
  }
  ~\label{fig:designing_data}
\end{figure}

==> 06-case-study.tex <==
\section{Case Study: Reflecting on Our Data Collection Process}
\label{sec:case-study}



It was unclear how diverse IMU data would influence our modeling experiments, or if the categories developed through our reflexive prompts would meaningfully align with variation within the data. Prior work on human gestures has shown age ~\cite{lee2020clip}, emotion ~\cite{noroozi2018survey}, and health \cite{8941232} influence gesture presentation.
Hand position during typing is similarly distinguishable \cite{goel2013contexttype}, yet IMU data collection rarely includes meta information about participants. Similarly, context is often not documented for image data (e.g. the proverbial question of \textit{what's outside the frame?}).



The results of \textit{Collection Monitoring} led to three instances of additional, retargeted data collection efforts based on unexpected skew. During our initial data collection, there were multiple categories which did not match our previously described distributions.
While all participants were employees from a large tech company, we did not anticipate our initial wave of data collection to be so skewed towards individuals between the ages of 21 and 40. In truth, we initially had no participants over 38. 
As a result, we emphasized diversity in participant age moving forward with some success---each consecutive wave improved the data coverage. Familiarity also directed our collection efforts, leading us to seek additional data for an intersectional subset of \texttt{Female} participants with \texttt{Large} phones and \texttt{Small} hands.







\label{sec:auditing}
